Search-Based Software Engineering for Self-Adaptive Systems: Survey, Disappointments, Suggestions and Opportunities

Search-Based Software Engineering (SBSE) is a promising paradigm that exploits the computational search to optimize different processes when engineering complex software systems. Self-adaptive system (SAS) is one category of such complex systems that permits to optimize different functional and non-functional objectives/criteria under changing environments (e.g., requirements and workload), which involves problems that are subject to search. In this regard, over years, there has been a considerable amount of work that investigates SBSE for SASs. In this paper, we provide the first systematic and comprehensive survey exclusively on SBSE for SASs, covering papers in 27 venues from 7 repositories, which eventually leads to several key statistics from the most notable 74 primary studies in this particular field of research. Our results, surprisingly, have revealed five disappointments that are of utmost importance and can result in serve consequences but have been overwhelmingly ignored in existing studies. We provide theoretical and/or experimental evidence to justify our arguments against the disappointments, present suggestions, and highlight the promising research opportunities towards their mitigation. We also elaborate on three other emergent, but currently under-explored opportunities for future work on SBSE for SASs. By mitigating the disappointments revealed in this work, together with the highlighted opportunities, we hope to be able to excite a much more significant growth in this particular research direction.

==> legacy.tex <==
\section{Disappointed Issues}
\label{sec:dis}
%what it has been doen in SAS, and how it should be done in EC/other field (some thing has been done, but could have been done better)
In this section, we present in-depth discussions of the disappointed issues derived from the survey results, together, supported by justifiable evidence.



  

% 1. unexplored algorithms
\subsection{Unjustified Bias on the Selection of Search Algorithms}

% number of considered algorithms in a paper:
% the top 10 considered algorithm and year of publication:

The long history of Computational Optimization community has witnessed a wide range of effective search algorithms. The other problems in SBSE have also attempted to explore various search algorithm over the last decade~\cite{DBLP:journals/tse/RamirezRS19}. However, as discussed in Section~\ref{sec:rq2} it is disappointed to find that when investigating SBSE for SASs, there is an unjustified bias on the selection of search algorithms, i.e., GA and ES are predominated for single or aggregated objective case; NSGA-II is significantly more common in Pareto-based multi-objective cases. 

  \begin{figure}
  \centering
  \begin{subfigure}[t]{0.5\columnwidth}
\includestandalone[width=\columnwidth]{tikz/femosaa-moead}
%\subcaption{level 3}
    \end{subfigure}
    \caption{Optimization results by MOEA/D-STM and NSGA-II for an example SAS over all runs~\cite{DBLP:journals/tosem/ChenLBY18}.}
  \label{fig:search-alg}
  %  \vspace{-0.7cm}
  \end{figure}
  
    \begin{figure}
    \centering
\includestandalone[width=0.5\columnwidth]{tikz/single-better-ga}
%\subcaption{level 3}
    \caption{Optimization results by Memetic Algorithm (MA) and GA for an example SAS over all runs~\cite{DBLP:journals/tsc/LeitnerHD13}.}
  \label{fig:search-alg-single}
  %  \vspace{-0.7cm}
  \end{figure}
  
Indeed, certain search algorithms are `better known' than some others, but such a large bias is what we did not expect. In fact, the selections have not been well-justified: undoubtedly, ES will not work for those widely used subject SASs with an explosion of search space, as shown in Section~\ref{sec:rq6}. While both GA and NSGA-II are arguably one of the most popular algorithms out of their own category, there has been no scientific evidences to prove that they are universally fit to all contexts, especially considering that the dynamics and uncertainty are heavily involved in the search problems of SAS. In particular, given the extremely active research within the computational optimization domain, it is possible that alternative algorithms perform much better for SAS optimization, which is not uncommon in other SBSE problems. For example, in the software product line optimization problem, IBEA~\cite{Zitzler2004} has been shown to be able to find solutions with better convergence and diversity than NSGA-II. This is also highly plausible on SAS problems. For example, a recent work on SBSE for SASs~\cite{DBLP:journals/tosem/ChenLBY18} has shown that MOEA/D-STM~\cite{DBLP:journals/tec/LiZKLW14}, which is a relatively new search algorithm proposed in 2015, tends to achieve better results than NSGA-II in terms of optimizing two conflicting objectives on different SASs that require configuration based self-adaptation. An example result has been shown in Figure~\ref{fig:search-alg} where the points that closer to the top-left region are the ideal adaptation solutions. Another work by Leitner et al.~\cite{DBLP:journals/tsc/LeitnerHD13} has also demonstrated that when configuring different SASs, the GA is inferior to MA, which is an even older search algorithm introduced in 1999, as shown in the example from Figure~\ref{fig:search-alg-single}.



  
    
    \begin{figure}[!t]
  \centering
\includestandalone[width=0.6\columnwidth]{tikz/alg-number-pie}
    \caption{Distribution on the number of search algorithms considered (with reported results) in the primary studies.}
 \label{fig:alg-pie}
  \end{figure}


In general, 
there are two issues leading to this disappointment. 
The first is that the number of search algorithms considered (with reported results) in each study is rather small, 
as can be seen in Figure~\ref{fig:alg-pie}. 
In particular, 
we see that there are as much as 63\% of the primary studies consider and present the results for only one search algorithm, 
and a further 15\% studies discuss two. 
This has already constituted to more than three quarters of the work surveyed. 
Such number apparently cannot be considered as a sufficiently wide exploration that covers the full spectrum of the possibility of SBSE for SASs. 
In fact, 
it is essential to `try' a good range of alternative search algorithms and report the results,
especially when the knowledge of the problem is not very clear. 
In the Computational Optimization and Evolutionary Computation community, 
it is not uncommon to investigate between four to six algorithms for majority of the work\footnote{Excluding empirical studies where the number of the compared algorithms may easily be over a dozen.}, 
in order to fully evaluate the effectiveness of the proposed approach and justify the choice. 
This has also been becoming a standard practice in SBSE. 
For example, 
on the test case generation~\cite{pradhan2018cbga} and refactoring~\cite{DBLP:journals/tse/LuWYAN19} problem, existing work (excluding empirical studies) has also studied and presented results based on three or more competitive search algorithms. Sometimes, there can be nine search algorithms~\cite{DBLP:journals/jss/ZhangAY19}.


%There are two fundamental issues underpin this disappointment, depending on whether a thorough understanding about the SAS problems (e.g., information about the search/objective space) and the search algorithms is available. When such an in-depth understanding is difficult, if not impossible, then it is essential to `try' a good range of alternative search algorithms on SBSE for SASs. This leads to our first issue, which, as clearly depicted in Figure~\ref{fig:alg-pie}, is that the number of search algorithms considered in each study is rather small. In particular, we see that there are as much as 63\% of the primary studies consider only one search algorithm, and a further 15\% studies consider two. This has already constituted to more than three quarters of the work surveyed. Such number, however, cannot be considered as sufficiently wide exploration that covers the full spectrum of the possibility of SBSE for SASs. In the Computational Optimization and Evolutionary Computation community, it is not uncommon to investigate between four to six algorithms for majority of the work\footnote{Excluding empirical studies where the number of the compared algorithms may easily be over a dozen.}, in order to fully evaluate the effectiveness of the proposed approach and justify the choice. This has also been becoming a standard practice in SBSE. For example, on the test case generation~\cite{pradhan2018cbga} and refactoring~\cite{DBLP:journals/tse/LuWYAN19} problem, existing work (excluding empirical studies) has also conducted experimental evaluation based on more than three competitive search algorithms. Sometimes, there can be 9 search algorithms~\cite{DBLP:journals/jss/ZhangAY19}


Another (probably more important) issue is to select search algorithms for comparisons according to the properties of the problem considered. 
It is known that every algorithm does have their own ``comfort zone''. 
But people tend to work by analogy; 
that is, using the algorithm which was (widely) used before. 
This may cause the risk of not being fully aware of their limitations. 
For example, 
ES is apparently not workable on large scale SASs;
GA may not be suitable for time-critical SASs; 
NSGA-II typically does not work on SAS problems with four and more objectives~\cite{Purshouse2007}. 
Therefore, 
selecting an algorithm suitable for the considered SAS problem is crucial, 
which demands a well understanding of both the problem and the algorithm. 
This, however, can emerge as a future opportunity on SBSE for SASs, 
as we will discuss in Section~\ref{sec:alg-sel}.

We therefore urge the researchers and practitioners in SBSE for SASs to consider a much wider and deeper investigation on the different search algorithms, as well as a more scientifically justifiable selection of algorithms based on the understanding between SAS problems and search algorithms where possible. 

%When both the SAS problems and the search algorithms can be well-understood, then our second issue is related to the lack of systematic and justifiable selection methodology of search algorithm(s) to be compared on SBSE for SASs. Such selection, however, is non-trivial and can emerge as a future research opportunity on SBSE for SASs, as will discuss in Section~\ref{sec:alg-sel}.

%why it is important, what is the issue


%Indeed, our reviews show that in a limited amount of the recent work on SBSE for SASs, a few previously unexplored search algorithms have been studied in SAS (e.g., MOEA/D-STM~\cite{DBLP:journals/tosem/ChenLBY18} and novelty search~\cite{DBLP:conf/saso/FredericksGK019}), and a relatively larger set of alternatives (i.e., up to 6) have been compared. However, this is still a rather small proportion with in the large amount of SBSE for SASs work, and therefore we urge the researchers and practitioners in this particular thread of research to consider a much wider and deeper investigation on the different search algorithms, as well as a more scientific selection of algorithms based on the understanding between SAS problems and search algorithms where possible. 

% 2. better synergise with the SE and SAS knolwedge, i.e., the need of engnieers

\subsection{Limited Synergy between Domain Knowledge and Search Algorithm}

% type of domain knowledge considered in the search per paper:

Given the very nature of the optimization involved in engineering SASs, exploring SBSE, or more generic sense of search algorithms, for SASs is certainly not new. Yet, disappointingly, from Section~\ref{sec:rq3}, we have failed to see how the advances of SBSE for SASs can be differed from ``another application domain of the search algorithms'', as 79\% of the primary studies merely specialize the search algorithm with the nature information about the problem. 

Since SBSE is relatively new to SAS research, this result is predictable, but we did not expect such a significant discrepancy. The key challenge that underpins this disappointment is how to exploit the expertise and domain knowledge of engineers to tailor which aspects of the search algorithms, in order to reach better specialized and improved optimization results. This is perhaps a more general issue on a wider context of SBSE problems, but there has been some very successful attempts in capturing and synergizing such knowledge into the algorithms on other SBSE research. For instance, for the software testing problems addressed by SBSE, the search algorithms are often manipulated to work with various types of seeds, which were specifically designed to match the contexts of the code to the test bed~\cite{DBLP:conf/icst/FraserA12}. There are also a considerable amount of work that focuses on specializing the operators of search algorithms to better serve the context~\cite{DBLP:conf/gecco/WuWHJK15}\cite{DBLP:journals/asc/XueZT0CC016}. 

%Note that here we refer to more than simply designing the representation of solutions and/or fitness evaluation, as these are the tasks that one would have to do in order to investigate SBSE for a problem. Rather, we keen to see additional tailoring of the search algorithms, derived from strong software and system engineering knowledge, to achieve better optimization for SAS. 

Ignoring the strong domain knowledge from engineers is a non-trivial issue on SBSE for SASs and can be an unwise waste of such valuable knowledge. For example, a recent work by Chen et al.~\cite{DBLP:journals/infsof/ChenLY19} on SBSE for SASs has shown that, instead of allowing the algorithm to search from scratch, seeding the search algorithm with high quality seeds, which were selected based on engineers' expertise, can largely improve the optimization result (i.e., the HV value) when configuring 10 different service-based SASs. An example\footnote{The work assumes that there is no preference towards any of the objectives, and thus hypervolume serves as a fair indicator on the overall quality of solution set.} has been illustrated in Figure~\ref{fig:search-knowledge}.

  \begin{figure}
  
  \begin{subfigure}[t]{0.45\columnwidth}
\includestandalone[width=\columnwidth]{tikz/w7-hseed-HV-nsgaii}
\subcaption{NSGA-II}
    \end{subfigure}
    ~
      \begin{subfigure}[t]{0.45\columnwidth}
\includestandalone[width=\columnwidth]{tikz/w7-hseed-HV-ibea}
\subcaption{IBEA}
    \end{subfigure}

  
    \caption{Mean hypervolume values for an example SAS with and without additional domain knowledge over all runs~\cite{DBLP:journals/infsof/ChenLY19}.}
  \label{fig:search-knowledge}
  %  \vspace{-0.7cm}
  \end{figure}
  
  
    


%why it is important, what is the issue

As shown in Section~\ref{sec:rq3}, we do see a few very good example work (e.g., \cite{DBLP:journals/tosem/ChenLBY18}\cite{DBLP:conf/icse/CailliauL17}\cite{DBLP:journals/infsof/ChenLY19}\cite{DBLP:conf/gecco/HaraldssonWBS17}) on better synergizing domain expertise and search algorithms when exploring SBSE for SASs, which constitutes to the renaming 21\% of the primary studies. This, as shown in those 21\% work, is in fact a win-win strategy, where on one hand, the search algorithm can be potentially made more controllable and explainable, on the other hand, the strong domain knowledge can serve as strong guidance to steer the search, achieving results that would be otherwise difficult to obtain. Further, the nature of complexity in SAS can actually provide more opportunity to design a better tailored and specialized search algorithm for the context. 

We therefore seek to increase the 21\% of primary studies and urge the community that when investigating SBSE for SASs, a better and more thorough synergy between domain knowledge and the search algorithms should be carefully considered. This disappointed issue also raise the need of highly specialized search algorithm that considers the characteristics of the algorithm itself; and human centric SBSE for SASs, in which the human (engineers) is permitted to control the search algorithms, rendering the results more explainable. We will further discuss these new opportunities for future research in Section~\ref{sec:alg-sel} and ~\ref{sec:hc}, respectively.



% 3. MOO
\subsection{Limited and Inaccurate Definition of Multi-Objective Search for SAS}
\label{sec:dis3}
% Relation between objective per paper:

Multi-objective search, in the context of Computational Optimization community and other SBSE problem, refers to simultaneously optimizing multiple (usually conflicting) objectives, thus resulting in a set of trade-off solutions, called Pareto optimal solutions. Searching for all Pareto optimal solutions (or a good approximation of them) provides the engineers with diverse choices from which they can choose their preferred one, but also with the knowledge/information of the optimization problem (e.g., correlation between the objectives, actual dimensionality of the Pareto front, and the location of knee points) for better understanding of the problem.

However, as shown in Section~\ref{sec:rq4}, our review discovers that on SBSE for SASs, the multi-objective search can refer to the fact that there are multiple conflicting objectives, but they are optimized in certain form of aggregation (i.e., weighted sum or product). We were disappointed to see that, this form of optimization is predominantly referred to as multi-objective search and constitutes to 52 primary studies, compared with 20 others that rely on the alternative, and perhaps more accurate way of multi-objective search using Pareto-based relation.


  \begin{figure}
  
  \begin{subfigure}[t]{0.45\columnwidth}
\includestandalone[width=\columnwidth]{tikz/single-op}
\subcaption{GA for equal weights}
    \end{subfigure}
    ~
      \begin{subfigure}[t]{0.45\columnwidth}
\includestandalone[width=\columnwidth]{tikz/multi-op}
\subcaption{NSGA-II}
    \end{subfigure}

  
    \caption{Comparing results by search with equally weighted objective aggregation (GA) and Pareto-based multi-objective search (NSGA-II) on the bi-objective DTLZ2 function.}
  \label{fig:single-vs-mutiple}
  %  \vspace{-0.7cm}
  \end{figure}

In essence, the aggregation of objectives implies that certain preferences over the objectives are available and they can be precisely quantified using weights, as we showed that the majority of them have either assumed the weights can be provided by the engineers or they are equally weighted by default. Indeed, if this is the case, then the aggregation way of search-based optimization can be ideal. However, it is not uncommon that a precise quantification of the weights are very difficult, if not impossible, especially given the complexity of SAS. In particular, despite being adopted in 20 primary studies, it is in fact an inaccurate assumption that setting equal weights to the objectives implies an equal importance and thereby leading to a fair solution, because the search pressure guided by the weighted fitness and a single objective search algorithm may not be able to discover certain solutions in the first place. For example, in Figure~\ref{fig:single-vs-mutiple}, we compare the case of searching with equally weighted sum of objectives (GA) and the Pareto-based multi-objective search (NSGA-II) on DTLZ2, a well-known bi-objectives test function from the Evolutionary Computation community. Clearly, after very few generations (less than 20), the GA converges to a single point while the NSGA-II produces a much more diverse set of Pareto optimal solutions, finally representing a full spectrum of the trade-off surface in the problem. It is interesting to note that, even equal weights have been given to the two objectives under the same scale, the final solutions are far from being balanced. In fact, it shifts towards the extreme where one objective is preferred more, i.e., close to the boundary points of the problem's Pareto front. This has apparently contradicted with the general belief that equally weighted objectives represent fair importance. The fundamental cause of this is that (i) the boundary points have higher aggregated fitness than inner points due to the concave shape of the Pareto front, and (ii) the gene drift phenomenon in GA easily lead the population to converge into one point. 



%In next section, the quality indicators used to assess the adaptation solution(s) when will be elalbrated into more details.

%\footnotetext{Some primary studies consider both at the same time.}.

%why it is important, what is the issue

The minority of the Pareto-based multi-objective search on SBSE for SASs, on the other hand, does not require weights specification during the search, which precisely addresses the shortcoming of weighted sum and product of the objectives. However, one challenge of Pareto-based multi-objective search is how to select a single solution from the produced nondominated trade-off set. When no preference information is available, it is ideal to provide the engineers with all nondominated solutions found to keep them informed in the decision-making process. When certain preferences exist, the selection of the single solution can be tailored with such. Yet, unlike the case of weighted aggregation, such preferences do not require explicit quantification. As we have shown in Section~\ref{sec:rq4}, this can be achieved with human intervention when possible (14 studies), or automatically completed by selecting a solution from certain regions, e.g., the knee point selection.

In our review, we have also observed that certain work apply both, e.g.,~\cite{DBLP:conf/icse/Garcia-GalanPTC14}\cite{DBLP:journals/tmc/PaolaFGRD17}, in which the search is conducted in a Pareto-based multi-objective way while the final solution is selected using one single weighted aggregation. This is an approach that we are particularly against, as it arises a clear contradiction: the fact that the weighted aggregation is used implies that certain preferences over the objectives are available and can be quantified, which contradicts with the fact that Pareto-based multi-objective search is usually conducted when such a clear quantification does not exist. Sadly, those studies have not explicitly discussed the rationals behind the choice. 

As a result, Pareto-based multi-objective search is what should be investigated more, at least in a comparative amount of attentions to the weighted aggregation, when exploiting SBSE for SASs. With this regard, a future direction on how to capture and model preference on SBSE for SASs has emerged as a new research opportunity, as we will discuss in Section~\ref{sec:cap-pref}.
%\textcolor{red}{To Miqing and Ke: could you please check and amend this part if needed?}


% 4. quality indicator
\subsection{Unjustified Quality Indicator Selection under Multiple Objectives}

% Top 10 considered QI in each paper:
% The aspect of information provided by each QI:


\begin{table}[t!]
	 \begin{threeparttable}
		\caption{The prerequisite and characteristics of the top 5 quality indicators considered in the primary studies.}	
		
	        \label{table:single-multi}	
	        \begin{tabularx}{\columnwidth}{P{2.2cm}|P{1.72cm}|Y|Y}\hline
		%\begin{tabular}{c|c|c|c|c|c}\hline
			& \textbf{\emph{utility}} & \textbf{\emph{objective value}} & \textbf{\emph{HV, IGD, $\epsilon$ and GD}}\\\hline
			\textbf{\emph{Prerequisite}}&  Preference on objectives& None & None   \\\hline
			\textbf{\emph{Comparing the solution(s) on all objectives?}} & Yes & No & Yes   \\\hline
			\textbf{\emph{Comparing solution sets?}} & No & No & Yes   \\\hline
			%Comparing solution sets&  & & $+$   \\\hline
		\end{tabularx}	
		 %\begin{tablenotes}
      %\footnotesize
      %\item ``$+$'' means that the indicator can collectively assess solution(s) on all objectives and 
			%``$-$'' means that the indicator can only assess solution(s) on individual objective.
    %\end{tablenotes}
	\end{threeparttable}
\end{table}


When multiple conflicting objectives of the SAS are involved, we have shown in Section~\ref{sec:rq5} that using utility or the value for each objective individually are predominated ways to assess the quality of solutions. Despite their popularity, it is disappointed that our review finds no systematic justification on the choice of utility and objective value as quality indicators for multiple objectives. This is important, because as shown in Table~\ref{table:single-multi}, the utility can collectively assess all objectives of a single solution only under the assumption that preferences are available and can be precisely quantified. However, as mentioned, it is not uncommon in SAS optimization that the preferences are not available or too difficult to be quantified. The objective value, on the other hand, is exempted from such prerequisite but only provides assessment on a single objective at a time. This is apparently not accurate as it ignores the quality of the solutions on other objectives. When there is a need to assess a solution set, such a way of considering objectives separately may lead to a situation that a solution set is evaluated better than another on all objectives individually, but it turns out that the engineer would never prefer it under any circumstance. The other quality indicators, e.g., HV, IGD, $\epsilon$-indicator and GD, are exactly designed to compare the solution set as a whole and have no prerequisite/preferences, but they have disappointedly attracted much less attention when compared with the utility and objective value.







In the Computational Optimization and Evolutionary Computation community, over hundreds of quality indicators have been proposed to assess the solution sets \cite{DBLP:journals/csur/LiY19}. Yet, we are disappointed to see that the work on SBSE for SASs has only explored a very limited set of them, as discussed in Section~\ref{sec:rq5}. It is with an even greater disappointment to discover that their selections also lack a systematic justification, but are driven by the facts that other work has also used the same ones. The issue here, however, is that each quality indicator has its own unique preferences. The one fitted well in other situations may not be suitable for the SAS problem. Even for two indicators which are designed for assessing the same quality aspect of a solution set, they could have very different preferences~\cite{DBLP:journals/csur/LiY19}. For example, both HV and IGD are used to provide a comprehensive evaluation of a solution set in terms of convergence, spread, uniformity and cardinality, but HV clearly prefers knee points of the Pareto front and IGD prefers uniformly-distributed solutions. Therefore, a careful selection and use of quality indicators have to be made to evaluate/compare solution sets since quality indicators can easily mislead the decision maker, returning opposite evaluation results to actual preferences of the decision maker ~\cite{DBLP:journals/csur/LiY19}\cite{DBLP:conf/icse/Li0Y18}.

For example, when reasoning about adaptation solutions, two common but conflicting objectives to be optimized can be the dependency compliance and the incurred cost\footnote{The actual meaning of cost depends on the context, e.g., it could be the time or resources required to realize adaptation.}: an adaptation solution with lower cost could likely to have a larger violation of the dependency. Let us assume two solution sets \texttt{A} and \texttt{B} in Figure~\ref{fig:qi-example} returned by two search algorithms. To compare these two sets, a typical practice is to consider one or several commonly-used quality indicators. Here, eight most commonly used quality indicators in SBSE are given in Table~\ref{table:taxonomy}, along with what quality aspects they can cover. As we can see, there are some indicators or their combinations which can (partially) cover all quality aspects of solution sets, thus being expected to give reliable evaluation. However, the fact is quite opposite --- all the eight indicators evaluate \texttt{A} better than \texttt{B}, but the decision maker may typically prefer the latter. This is because, in this particular context, the dependency needs to reach 100\% compliance or otherwise an adaptation solution is considered as invalid, which cannot be used to adapt the software system at all. The solution ($\beta$) of \texttt{B} reaches 100\% and has lower cost than the corresponding one in A, which should have been the most ideal solution. This is a typical example that indicates the risk of directly using existing quality indicators without considering the nature/preferences of the problem~\cite{DBLP:conf/icse/Li0Y18}.


%The issue here, however, is that each quality indicator only assess one or certain aspects of a solution set (e.g., convergence, uniformity and spread etc)~\cite{DBLP:conf/icse/Li0Y18}. A summary of the most widely used quality indicators for solution sets in SBSE, as well as what quality aspects they cover, have been shown in Table~\ref{table:taxonomy}. As we can see these quality indicators offer diverse aspects of information, the selection of those quality indicators therefore should be made with respect to the quality of aspects they cover, whether these aspects are important to the problem and whether they should be assessed individually or collectively. 


%Additionally, the selection of indicator for solution sets should be aligned with the needs of the contexts and preferences (if available). For example, as depicted in Figure~\ref{fig:qi-example}, two common objectives to be optimized when reasoning about adaptation can be the dependency compliance and the incurred cost\footnote{The actual meaning of cost depends on the context, e.g., it could be the time or resources required to realize adaptation.}: an adaptation solution with lower cost could likely to have larger violation of the dependency. A possible result of two solution sets \texttt{A} and \texttt{B} has been shown in Figure. However, in this case, if the common indicators (e.g., HV and IGD) are used, it would lead to an inappropriate conclusion such that \texttt{A} is better than \texttt{B}. This is because, in this particular context, the dependency needs to reach 100\% compliance or otherwise an adaptation solution is considered as invalid, which cannot be used to adapt the software system at all. In fact, the particular solution $\alpha$ in set \texttt{B}, which reaches 100\$ compliance, is the one that should be used. Similar issue can occur in case where one objective is preferred over the others, but it is unclear about how much exactly such objectives is favored more.





%why it is important, what is the issue, it is also possible that one objective is more important, but do not know how much more important.
% exp 1: information about prefer dependency exp vs cost 2: information about prefer an objective over the others





In fact, the lack of systematic justification on the selection of quality indicators when using SBSE for multi-objectively optimizing SAS is also an overwhelming problem in the entire SBSE domain~\cite{DBLP:conf/icse/WangAYLL16}\cite{DBLP:conf/icse/Li0Y18}, but it is of particular importance on SBSE for SASs, given the wide variety of possible objectives to be optimized.  

Based upon the above discussion, we urge the community on this thread of research to carefully consider the selection of multi-objective quality indicators, which itself could potentially be a promising research area. This disappointed issue is again related to the new research opportunity of how to capture and model preference on SBSE for SASs, which we will discuss in Section~\ref{sec:cap-pref}.

%\textcolor{red}{To Miqing: could you please check and amend this part if needed?}


\subsection{Weak Generalization of Results across the Subject SASs}

% The number of considered subject SAS per paper:
% The number of considered subject SAS that is of different type per paper:

% 5. generaization issue in the subject SAS
In Section~\ref{sec:rq6}, we have shown that a variety of subject SASs are considered on SBSE for SASs. Yet, disappointedly, our review has indicated that there are 65\% primary studies consider only one SAS, and 87\% consider less than three. It becomes even more disappointed if we differentiate the SASs based on their domains, as discussed in Section~\ref{sec:rq6}, where the portion of studies that considers one SAS increases to three quarters, with the number of studies that consider less than three subject SASs increase to 97\%. From the research work on other SBSE problems, it is not uncommon to see a wide range of subject software systems have been used (even excluding empirical studies), for example, SBSE for software product line engineering often involve more than 10 distinct subject systems~\cite{DBLP:journals/asc/XueZT0CC016}. In the Computational Optimization and Evolutionary Computation community, the number of test functions used to evaluate a search algorithm is also most commonly to be more than 10 (excluding empirical studies). Comparatively, the number of subject SASs considered is current work on SBSE for SASs is rather limited, even when pure empirical studies are included.

\begin{table}[t!]
	 \begin{threeparttable}
		\caption{The median GD (IQR) produced by NSGA-II and SPEA2 when search on different SASs from distinct domains over all runs~\cite{DBLP:journals/jss/PascualLPFE15}.}	
		
	        \label{table:subject-example}	
	        \begin{tabularx}{\columnwidth}{Y|Y|Y}\hline
		%\begin{tabular}{c|c|c|c|c|c}\hline
			  &\textbf{\emph{NSGA-II}}&\textbf{\emph{SPEA2}} \\\hline
			  \textbf{\emph{x264}} &\cellcolor{yellow}0.00{\footnotesize(0.00)}&\cellcolor{yellow}0.00{\footnotesize(0.00)} \\\hline
			  \textbf{\emph{Wget}} &0.91{\footnotesize(2.7E+2)}&\cellcolor{yellow}0.74{\footnotesize(2.6E+2)} \\\hline
			  \textbf{\emph{Berkeley}} &0.22{\footnotesize(5.6E+2)}&\cellcolor{yellow}0.00{\footnotesize(4.4E+2)} \\\hline
			  \textbf{\emph{Sensor}} &\cellcolor{yellow}1.23{\footnotesize(1.9E+3)}&1.29{\footnotesize(1.4E+3)}\\\hline
			  \textbf{\emph{Game}} &2.41{\footnotesize(1.7E+3)}&\cellcolor{yellow}2.19{\footnotesize(1.4E+3)}\\\hline
			  \textbf{\emph{Tank War}} &\cellcolor{yellow}2.08{\footnotesize(6.7E+2)}&2.09{\footnotesize(6.3E+2)}\\\hline
			  \textbf{\emph{Media}} &2.96{\footnotesize(1.2E+3)}&\cellcolor{yellow}2.90{\footnotesize(1.1E+3)} \\\hline
			  \textbf{\emph{Guide}} &\cellcolor{yellow}1.58{\footnotesize(3.8E+2)}&1.72{\footnotesize(3.7E+2)} \\\hline
		\end{tabularx}	
		 \begin{tablenotes}
      \footnotesize
      \item The better one is highlighted.
    \end{tablenotes}	
	\end{threeparttable}
\end{table}

This can be a crucial issue when conducting research on SBSE for SASs, as it weakens the generalization of the conclusion drawn. An example from Pascual et al.'s work~\cite{DBLP:journals/jss/PascualLPFE15} has been shown in Table~\ref{table:subject-example}, in which the GD results produced by the search algorithms on configuring 8 different SASs are compared. It is unclear to claim whether NSGA-II or SPEA2 can generally outperform the other as they are competitive across all the SASs. However, if only limited subject SASs are considered, it is possible that \texttt{Sensor}, \texttt{Game} and \texttt{Guide} may be chosen, which would lead to an inappropriate conclusion such that NSGA-II is generally better. Therefore, we urge the community to consider more subject SASs in future work on SBSE for SASs. Of course, arguably the setup and deployment of working SASs can be more complex than the systems in other SBSE problems, but those subject SASs need not to be real software systems; they can well be simulators, e.g., those prototyped artifacts from the SEAMS artifacts track\footnote{https://www.hpi.uni-potsdam.de/giese/public/selfadapt/ exemplars/}.

%a recent work on optimizing adaptable systems has also considered 15 systems []. However, as shown in Table~\cite{table:subject-example}, we were disappointed to see that most of the work on SBSE for SAS has only considered one subject software systems.

  

  
%why it is important, what is the issue



\section{Opportunities}
\label{sec:opp}
%new directions, potentially to further advance the field (soemthing that has not been done, or not being done properly)

Despite of having several disappointed and overwhelming issues, SBSE for SASs is still a vital research direction which also bears many opportunities. In this section, we specify those opportunities and outline their promising research directions, as well as the related challenges to be addressed.

\subsection{Justifiably Selecting Search Algorithm according to Problem Instances on SBSE for SASs}
\label{sec:alg-sel}
%\textcolor{red}{To Miqing: could you please add some texts on this part?}

An interesting phenomenon in SAS as well as SBSE is that in spite of the considerably large number of search algorithms currently available, 
the primary studies adopt/compare just very few of them, as we shown in Section~\ref{sec:rq2}. 
Several algorithms have a clear preference, 
such as GA and ES for a generic optimization case and 
NSGA-II for the multi-objective optimization case.
Indeed, 
every search algorithm has their own merit,
which makes them well-suitable to a particular class of problems.
For a generic optimization case, 
it is clear that if the scale of the problem is small enough to allow enumerating all solutions (with a given time budget),
then ES can be a good option as it can guarantee the optimal solution. 
Some algorithms are designed for a particular class of problems, 
and it is expected that these algorithms may produce better solutions than algorithms designed for generic problems, 
for example Branch and Bound (BB) for some combinatorial problems.
The algorithms RS, Greedy Search (GS), HC and GA cannot guarantee an optimal solution.
As its name suggests, 
RS visits the space randomly and the final solution can be rather different in each run of the algorithm.
As opposed to RS, every iteration (step) in GS is determined (to make the current optimal choice),
in order to the overall optimal way to solve the entire problem. 
HC may be deemed as a combination of RS and GS,
as it starts from a random initial point in the search space and 
iteratively finds out the best neighbor of the current solution. 
Compared to RS, GS and HS, 
GA (and other metaheuristics) is a sophisticated optimization algorithm.
Its population-based search strategy with a diversity preservation can help to some extent the search jump out of local optimum.
A particular benefit of such population-based search is dealing with multi-objective problems, where each individual in the population can be used to approximate a unique trade-off between objectives.

For the multi-objective case, 
as shown in Figure~\ref{fig:alg-count2}, 
most of the algorithms considered belong to GA or its variants.
Consequently, 
the range of problems that the algorithms are suitable for is narrow and overlapping. 
Nevertheless, 
different multi-objective GAs do have their own ``comfort zone''. 
For example, 
the algorithms which compare solutions by Pareto dominance and density, such as NSGA-II~\cite{DBLP:journals/tec/DebAPM02} and SPEA2~\cite{Zitzler2002}, 
typically do not work well on many-objective problems where the number of objectives is larger than three~\cite{Purshouse2007}. 
The decomposition-based algorithms (e.g., MOEA/D~\cite{Zhang2007} and its variants MOEA/D-STM~\cite{DBLP:journals/tec/LiZKLW14} and NSGA-III~\cite{Deb2014}) scale up well in terms of objective dimensionality, 
but may struggle on problems with an irregular Pareto front shape (e.g. degenerate, disconnect or highly-nonlinear)~\cite{Ishibuchi2017}.
The indicator-based algorithms (e.g., IBEA~\cite{Zitzler2004}) are often insensitive to the Pareto front shape, 
but may suffer from the dominance resistance solutions (i.e. solutions with an extremely poor value on at least one of the objectives but with (near) optimal values on the others~\cite{Ikeda2001}), thereby with their solutions concentrating in the boundaries of the Pareto front~\cite{Li2018}.

Overall, 
it is important to understand the behavior and advantages/drawbacks of search algorithms available, 
which, together with the problem knowledge, will certainly help to choose an appropriate algorithm that is well-suited to the problem in hand.
To achieve that, 
there are several challenging research questions desirable for us to address.

\begin{itemize}

\item What kind of information/knowledge of the SAS problem can be obtained/extracted, and how.

\item What kind of search algorithm can make better use of such information/knowledge, which can greatly inform the algorithm selection. 


\item Or further, how to generically develop a specialized search algorithm specifically for a SAS problem.  

\end{itemize}


\subsection{Capturing Preferences of the Engineers in SBSE for SASs}
\label{sec:cap-pref}
% Preferences refer to one's satisfaction on certain aspects of the SAS, and they can come from not only the software engineers, but also any stakeholders involved in the process of engineering SAS. \textcolor{red}{To Ke: could you please add some texts on this part?}

Preferences refer to one's satisfaction on certain aspects of the SAS, and they can come from the software and system engineers, who have specific software engineering expertise, and would make various decisions in engineering SAS. While preference exist even for the single objective case, it is of even greater importance when there are multiple conflicting objectives for the SAS. According to the software engineering expertise of the engineers, s/he might only be interested in a handful of selected solutions that meet their preference most, instead of the entire set of solution obtained by a Pareto-based multi-objective search algorithm. As a matter of fact, this has been a long standing topic in the Computational Optimization community over half a century.

As we discussed in Section~\ref{sec:rq4}, 14 primary studies on SBSE for SASs, which constitute to the majority, have captured preferences in \textit{a posteriori} manner, where a set of widely spread trade-off alternatives are obtained by a search algorithm before being presented to the engineers. However, this obviously increases the engineers' workload and will incorporate much irrelevant or even noisy information during the decision-making process. To alleviate the cognitive burden of the engineers, some pre-screen techniques have been introduced to help select a handful of representative solutions before handing over to the engineers. These, as shown in Section~\ref{sec:rq4}, include selecting only the knee point(s) or solutions that are significantly superior on certain preferred objectives. Indeed, \textit{a posteriori} manner mainly captures preferences based on the natural cognition of engineers rather than their software engineering expertise, as the captured preference cannot influence the search process.

The above has raised the research opportunity of SBSE for SASs on handling preference in \textit{a priori} or even an \textit{interactive} manner. In this regard, the former means that the preference information can also be elicited \textit{a priori} and is used as a criterion to evaluate the fitness that drives the search towards the region of interest along a pre-defined preferred direction. For example, the preference information can be represented as one or more reference points, each dimension of which represents the engineers' expectation at the corresponding objective~\cite{DebSBC06,LiCMY18}. Such information can be formally extracted from some software engineering design notations, such as the goal model. However, capturing the preferences only occur at the beginning of the search. The latter, i.e., the \textit{interactive} manner, permits continuous refinement of the preferences and thus allowing more accurate capture. Such an interactive preferences capture is a point we will further elaborate in Section~\ref{sec:hc}. To achieve \textit{a priori} or \textit{interactive} capture of preferences, there are several challenging research questions need to be addressed:
\begin{itemize}
    %\item How to enable the decision maker to engage with the search algorithm? This aspect is of the first priority as the decision maker cannot provide any useful information unless (s)he can understand the solutions at hand. It is worthwhile to investigate advanced visualization and human-computer interaction mechanisms to achieve this.
    \item How to automatically extract the stockholders' preference information in an efficient and cost effective manner.
    
    \item How to structuralize the preferences in a way that is understandable by the search algorithm.
    
    \item What parts of the stockholders' preferences, expressed in some software engineering representations, can be correlated to which quality aspect of the solution.
    
  
    
    %Different from the traditional machine learning problem, the training data are collected in a sequential manner and one cannot expect a large amount of the data available before conducting preference learning. It is interesting to consider techniques from active learning to help develop effective learning algorithms.
\end{itemize}

%It is not uncommon that there exist more than one objective in the process of engineering SAS. Instead of a set of trade-off solutions obtained by running an evolutionary multi-objective optimization algorithm, stakeholders might only be interested in a handful of selected solutions that meet their preference most. In this case, it is of practical importance to capture and take advantages of user preferences in SBSE for SASs. As a matter of fact, this has been a long standing  topic in the Computational Optimization community over half a century. There are three classes of hybrid techniques considering the synergy of optimization and MCDM: \textit{a posteriori}, \textit{a priori}, and \textit{interactive}.

%The most straightforward way is the \textit{a posteriori} decision-making where a set of widely spread trade-off alternatives are obtained by an evolutionary multi-objective optimization algorithm before being presented to the decision maker. However, this obviously increases the decision maker's workload and will incorporate much irrelevant or even noisy information during the decision-making process. To alleviate the cognitive burden of the decision maker, some pre-screen techniques have been introduced to help select a handful of representative solutions before handing over to the decision maker for MCDM. For example, in~\cite{DBLP:journals/tosem/ChenLBY18}, knee point(s) are used as the indicator to represent the solution(s) of interest to the decision maker.

%On the other hand, the preference information can also be elicited \textit{a priori} and is used as a criterion to evaluate the fitness of a solution in the environmental selection and to drive the population towards the region of interest along a pre-defined preferred direction. For example, the preference information can be represented as one or more reference points (or as known as aspiration level vectors), each dimension of which represents the decision maker's expectation at the corresponding objective~\cite{DebSBC06,LiCMY18}. However, it is worth noting that the decision maker can only interact with the algorithm once at the outset of the optimization process. It is controversial that the decision maker is able to faithfully represent her/his preference information beforehand.






\subsection{Effective and Efficient Fitness Evaluation in SBSE for SASs}
%\subsection{Better specialize current practice of optimization for SAS}
A crucial part of SBSE is how the fitness of a solution can be evaluated, which serves as the key to drive the search process. This, in the context of SASs, is often related to how the behaviors of the systems can be changed with different adaptation solutions. In certain scenario, it is possible to profile the SAS at design time, or at runtime where the profiling only affect the SAS in certain aspects rather than changing the whole system~\cite{DBLP:conf/icse/Gerostathopoulos18}. However, most commonly, such profiling is expensive and time consuming. In contrast, surrogate models that are based on machine learning has been explored as an alternative, given that they are relatively cheap in terms of the fitness evaluation as the search proceeds~\cite{DBLP:conf/icse/Chen19b}. Yet, this comes with the cost of high complexity in building such model, which may still be lack of accuracy or difficult to capture the up-to-date changes of SASs. Further, the amount of examples required to train the model can also hinder the effectiveness of the search.

The situation raises the research opportunity of investigating effective and efficient fitness evaluation in SBSE for SASs. In particular, the key difficulty lies in the question on how to keep the overhead of fitness evaluation low, while maintaining a reasonable accuracy and cost of building the surrogate model. A promising direction on this is the research area of incremental online learning, where the model can be learned with limited data samples and can be efficiently updated as new data is collected while providing adequate accuracy~\cite{DBLP:conf/icse/Chen19b}. The other possible direction is to explore so-called novelty model that does not required to observe the behaviors of SASs when using SBSE~\cite{DBLP:conf/kbse/RamirezJCK11}. Such a model mimics the natural phenomenon where the evolution would never be solely guided by explicit objectives, but also the biological novelty of the individuals. In such a way, the fineness can be assessed without the need to affect or acquire data from the SASs, and thus mitigating expensive evaluation. However, more research questions need to be addressed in order to better incorporate online learning with SBSE for SASs, such as the following: 

\begin{itemize}

\item Whether the frequency of model update could have an impact to the search results.

\item How to handle the trade-off between the cost of model building and the accuracy (or relevance) of the model, if any.

\item What are the correlations between the accuracy (or relevance) of a model to the improvement of SBSE for SASs.
%\item How accurate is deemed as sufficient such that being more accurate has no (or trivial) improvement to the SBSE for SASs.

\end{itemize}



%\subsection{SBSE and Control Theory for SAS}

%\subsection{SBSE and Verification for SAS}

%\subsection{SBSE and Machine Learning for SAS}

\subsection{Just-in-Time Handling of Changes in SBSE for SASs}

SAS would inevitably face with changes on the requirements, environment or its internal states, either at design time or at runtime. Despite the fact that SBSE is capable of naturally handling dynamics to some extents, the more fundamental problem is how often should the optimization runs in order to ensure that the results can cope with the new changes. Current researches on SBSE for SASs have almost ignored this point or simply assume that the search algorithm can be re-triggered when there is a need (e.g., according to a fixed frequency or upon the occurrence of changes). Yet, such a strategy would suffer the limitation that no changes can be captured during the run of the search algorithm.



To this end, recent advances on so-called dynamic optimization~\cite{DBLP:journals/swevo/NguyenYB12} and dynamic SBSE~\cite{harman2012dynamic} is a promising, but under-explored solution for SASs. Here, the key idea is to allow the search algorithm to automatically pick up any new changes during the search process, and therefore the new information can be used to steer the search or old and useless information can be discard in order to prevent misleading. Such a very nature is a perfect fit to various problems with `changes' that are faced by modern SASs. However, there are some crucial challenges on this particular direction of research on SBSE for SASs, for example:



 \begin{itemize}



 \item What are the mappings between the changes on SASs and the changes with respect to the search algorithm.



 \item What are the changes can be handled while the search is under processing, and how they can be fed into the search.



 \item Whether it is possible to generically consolidate any given search algorithm.



 \end{itemize}

\subsection{Human-Centric SBSE for SASs}
\label{sec:hc}
The main purpose of engineering SASs is to reduce the levels of human intervention on the running software systems. However, it has been shown that there are scenarios where human involvement is essential~\cite{DBLP:conf/icse/CamaraMG15}, or human knowledge has been proven to be able to greatly improve the behaviors of SASs. Similarly, SBSE is also motivated from the same origin: to automatically generate the software engineering process and thus free the software engineer from tedious and error-proven tasks. Recently, there is an ongoing demand to engineer human-centric SBSE, such that the search approach does not make the final decision on its own, but serving as an assistant to add insight for human to make decisions. Those two facts, together, imply a perfect match between the two fields in terms of the human-centric aspect.



In particular, human can refer to a wide range of engineers with certain software engineering expertise around SASs, including but not limited to, developers, requirements analyst, architects and testers. Among others, interactive SBSE, in which the human's domain knowledge of expertise can be used to explicitly control the search process with explainable outcomes, is a promising research opportunity for this thread of research. 

Specifically, the interactive SBSE is an emerging paradigm for decision making for software engineering problems on the fly. Combing together with the preferences capturing discussed in Section~\ref{sec:cap-pref}, interactive SBSE enables the human to progressively learn and understand the characteristics of the SAS problem at hand and adjust towards more appropriate capture of the preferences information. As a result, solutions can be gradually driven towards the region of interest~\cite{LiCSY18}, allowing the human to have more controllability over the search algorithm using their software engineering expertise~\cite{DebSKW10}. This would also create more inspirations to build specialized search algorithms, which should work the best under the SAS where the knowledge lies. Yet, the challenges can be related to:

%For example, in~\cite{LiCSY18}, during the optimization process, some selected solutions are presented to the software engineers for marking every several generations. Thereafter, the marked solutions are used as the training data to train a neural network to model the user preference which is used as the guidance in the optimization process. 

%Since the decision maker has a more frequent chance to provide new information, as discussed in~\cite{DebSKW10} the decision maker may fell more in charge and more involved in the overall \textit{optimization-cum-decision-making} process.

 \begin{itemize}

 \item What forms of human knowledge/expertise can explicitly influence which aspects of SBSE for SASs.


 \item How human can be placed in the loop in order to facilitate timely interaction with SBSE for SASs.



 \item How to ensure the information provided by human is reliable, i.e., how to prevent immature inputs.



 \end{itemize}

\subsection{Incorporating SBSE with Other Approaches for SASs}

SBSE would never be the sole approach for tackling problems in SASs. In fact, given the nature of ``optimization" implied in SBSE, there is a variety of opportunities to incorporate SBSE and other approaches for SASs, such as control theory, verification, machine learning and so forth. Our review has witnessed a few successful work that specifically incorporates SBSE with the other approaches, for example, Gerasimou et al.~\cite{DBLP:journals/ase/GerasimouCT18} have adopted SBSE, guided by probabilistic verification model, to search for optimal adaptation solution; Maggio et al.~\cite{DBLP:conf/sigsoft/MaggioPFH17} have also applied control-theoretic adaptation that is tuned using SBSE. However, there is a lack of general guideline about the possible forms of incorporation. This is important, especially given the wide applicability of SBSE and other approaches for engineering SASs. In particular, challenges can be raised by the following new directions of research:



 \begin{itemize}

 \item What are the patterns involved when incorporating SBSE with the other approaches for engineering SASs.

 \item Whether there could be a ``symbiotic" relation exist between SBSE and the another approach, i.e., both SBSE and the other can benefit from each other, which collaborates together to improve the SAS.

 \item How to codify a generic methodology that guides the practitioners of SASs on incorporating SBSE with the other approaches.



 \end{itemize}

==> tables/qi-preference.tex <==
\begin{table}[t!]
\centering
\caption{Assumed preferences between objectives and the used indicators on SBSE for SAS.}
\label{tb:qi-pref}
%\setlength{\tabcolsep}{7mm}{

\centering

\begin{tabular}{cc}\toprule
\textbf{Preference}&\textbf{Indicators}\hfill\\ 
\midrule

Clear&\\
Vague&-\\
Specific regions&\\
No preferences&\\



\bottomrule
\end{tabular}

\begin{tablenotes}
    \footnotesize
    \item Number in the bracket indicates how many studies are involved.
\end{tablenotes}
\end{table}

==> tables/venues-bk.tex <==
 
\begin{table*}[t!]
  \caption{The primary studies and their venues.}
  
\label{tb:papers-count} 
\begin{tabularx}{\textwidth}{p{8cm}P{1cm}P{1.5cm}P{0.5cm}Y}
\hline 
\multicolumn{1}{c}{\textbf{Journal}} &\textbf{Searched} & \textbf{Candidate} &\multicolumn{2}{c}{ \textbf{Primary}}
\\
\hline 
ACM Transactions on Software Engineering and Methodology & 4 & 1 & 1 &\cite{DBLP:journals/tosem/ChenLBY18} \\ \hline 
IEEE Transactions on Software Engineering & 69 & 21 & 8 &\cite{DBLP:journals/tse/CalinescuGKMT11}~\cite{DBLP:journals/tse/MalekMM12}~\cite{DBLP:journals/tse/CardelliniCGIPM12}~\cite{DBLP:journals/tse/RosaRLHS13}~\cite{DBLP:journals/tse/MoserRD12}~\cite{DBLP:journals/tse/EsfahaniEM13}~\cite{DBLP:journals/tse/NallurB13}~\cite{DBLP:journals/tse/WangHYY18} \\ \hline 
Elsevier Journal of Systems and Software& 170 & 28 & 8 &\cite{DBLP:journals/jss/VerbelenSSTD11}~\cite{DBLP:journals/jss/ChengG12}~\cite{DBLP:journals/jss/Potena13}~\cite{DBLP:journals/jss/PascualLPFE15}~\cite{DBLP:journals/jss/BashariBD18}~\cite{DBLP:journals/jss/CalinescuCGKP18}~\cite{DBLP:journals/jss/XuB19a}~\cite{DBLP:journals/jss/Gerostathopoulos19} \\ \hline
IEEE Transactions on Services Computing & 98 & 19 & 3 &\cite{DBLP:journals/tsc/LeitnerHD13}~\cite{DBLP:journals/tsc/SharmaR19}~\cite{DBLP:journals/tsc/ChenB17} \\ \hline 
IEEE Transactions on Cloud Computing & 100 & 13 & 1 &\cite{7523230} \\ \hline 
IEEE Transactions on Mobile Computing & 70 & 15 & 1 &\cite{DBLP:journals/tmc/PaolaFGRD17} \\ \hline 
Springer Service Oriented Computing and Applications & 41 & 7 & 1 &\cite{DBLP:journals/soca/HuberHKBK14} \\ \hline 
ACM Transactions on Autonomous and Adaptive Systems & 76 & 25 & 6 &\cite{DBLP:journals/taas/LewisECRTY15}~\cite{DBLP:journals/taas/Garcia-GalanPTC16}~\cite{DBLP:journals/taas/ZoghiSLG16}~\cite{DBLP:journals/taas/SuchR16}~\cite{kinneer2019information}~\cite{DBLP:journals/taas/ShevtsovWM19} \\ \hline 
Elsevier Information Science & 120 & 19 & 1 &\cite{DBLP:journals/isci/NascimentoL17} \\ \hline  
Springer Automated Software Engineering & 35 & 8 & 2 &\cite{DBLP:journals/ase/GerasimouCT18}~\cite{DBLP:journals/ase/DellAnnaDD19} \\ \hline 
Elsevier Information and Software Technology & 45 & 4 & 1 &\cite{DBLP:journals/infsof/ChenLY19} \\ \hline 
Elsevier Future Generation Computer Systems & 370 & 31 & 3 &\cite{DBLP:journals/fgcs/VerbelenSTD13}~\cite{DBLP:journals/fgcs/PascualPF15}~\cite{DBLP:journals/fgcs/BarakatML18} \\ \hline  
ACM Transactions on Parallel Computing & 2 & 1 & 1 &\cite{DBLP:journals/topc/BehzadBPS19} \\ \hline 
Proceedings of IEEE & 4 & 1 & 1 &\cite{DBLP:journals/pieee/TsigkanosMD19} \\ \hline 
\multicolumn{1}{c}{\textbf{\emph{Conference and Symposium}}}&\multicolumn{4}{c}{} 
\\
\hline
IEEE/ACM Conference on Software Engineering  & 310 & 17 & 1  &\cite{DBLP:conf/icse/ChenPYNZ14}\\ \hline 
IEEE Conference on Autonomic Computing & 290 & 13 & 3  &\cite{DBLP:conf/icac/RamirezKCM09}~\cite{DBLP:conf/icac/MorenoCGS16}~\cite{DBLP:conf/icac/GhahremaniG017}\\ \hline 
IEEE/ACM Conference on Automated Software Engineering & 230 & 22 & 2  &\cite{DBLP:conf/kbse/WangM09}~\cite{DBLP:conf/kbse/GerasimouTC15}\\ \hline 
IEEE Conference on Services Computing & 440 & 37 & 2  &\cite{DBLP:conf/IEEEscc/MiWYZSY10}~\cite{DBLP:conf/IEEEscc/JiangPLC12}\\ \hline 
ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering & 420 & 27 & 5  &\cite{DBLP:conf/sigsoft/ElkhodaryEM10}~\cite{DBLP:conf/sigsoft/EsfahaniKM11}~\cite{DBLP:conf/sigsoft/FilieriHM15}~\cite{DBLP:conf/sigsoft/ShevtsovW16}~\cite{DBLP:conf/sigsoft/MaggioPFH17}\\ \hline 
IEEE Conference on Requirements Engineering & 100 & 9 & 1  &\cite{DBLP:conf/re/PengCYZ10}\\ \hline 
IEEE/ACM Symposium on Software Engineering for Adaptive & 200 &42 & 12 &\cite{DBLP:conf/icse/PascualPF13}~\cite{DBLP:conf/icse/ChenB14}~\cite{DBLP:conf/icse/Garcia-GalanPTC14} ~\cite{DBLP:conf/icse/CamaraMG14}~\cite{DBLP:conf/icse/GerasimouCB14}~\cite{DBLP:conf/icse/FredericksDC14}~\cite{DBLP:conf/icse/HerbstKWG15}~\cite{DBLP:conf/icse/CailliauL17}~\cite{DBLP:conf/icse/KinneerCWGG18}\\  

and Self-Managing Systems&  &  &   &\cite{DBLP:conf/icse/Gerostathopoulos18}~\cite{8787163}~\cite{DBLP:conf/icse/JamshidiCSKG19}\\ \hline 

ACM Conference on Genetic and Evolutionary Computation& 320 & 5 & 3  &\cite{DBLP:conf/gecco/WuWHJK15}~\cite{DBLP:conf/gecco/HaraldssonWBS17}~\cite{DBLP:conf/gecco/0001LY18}\\ \hline 
IEEE Conference on Software Architecture & 30 & 3 & 1  &\cite{DBLP:conf/icsa/CalinescuCGKP17}\\ \hline 
ACM Conference on Systems and Software Product Line & 16 & 2 & 1  &\cite{DBLP:conf/splc/WeckesserKPMSB18}\\ \hline  
ACM Conference on Performance Engineering & 260 & 19 & 1  &\cite{DBLP:conf/wosp/0001BWY18}\\ \hline  
Springer Conference on Fundamental Approaches to Software Engineering & 90 & 6 & 1  &\cite{DBLP:conf/fase/CalinescuGB15}\\ \hline  
IEEE Conference on Self-Adaptive and Self-Organizing Systems & 140 & 31 & 2  &\cite{DBLP:conf/saso/FredericksGK019}~\cite{DBLP:conf/saso/PodolskiyMKGP19}\\ \hline  

\multicolumn{1}{c}{\textbf{Total}} & 3,740 & 409 & 73 \\ \hline  
\end{tabularx}
\end{table*}

==> tikz/exp/lit-rq5.tex <==
 \begin{table}[t!]
 
\centering
	\caption{The median GD(IQR) by NSGA-II and SPEA2 on different SASs of distinct domains over all runs from~\cite{DBLP:journals/jss/PascualLPFE15}.}
\label{tb:lit-rq5}
\setlength{\tabcolsep}{1.2mm}

\centering

\begin{tabular}{ccc|cc}\toprule

&\textbf{NSGA-II}&\textbf{SPEA2}&\textbf{NSGA-II}&\textbf{SPEA2}\hfill\\ 
\midrule


	  \textsc{Guide} &\cellcolor{yellow}1.58{\footnotesize(3.8E+2)}&1.72{\footnotesize(3.7E+2)}&\cellcolor{yellow}1.58{\footnotesize(3.8E+2)}&1.72{\footnotesize(3.7E+2)}\\
	  
  \textsc{Tank War} &\cellcolor{yellow}2.08{\footnotesize(6.7E+2)}&2.09{\footnotesize(6.3E+2)}&\cellcolor{yellow}2.08{\footnotesize(6.7E+2)}&2.09{\footnotesize(6.3E+2)}\\
  
			  \textsc{x264} &&&\cellcolor{yellow}0.00{\footnotesize(0.00)}&\cellcolor{yellow}0.00{\footnotesize(0.00)} \\
			  
			  \textsc{Wget} &&&0.91{\footnotesize(2.7E+2)}&\cellcolor{yellow}0.74{\footnotesize(2.6E+2)} \\
			  
			  \textsc{Berkeley} &&&0.22{\footnotesize(5.6E+2)}&\cellcolor{yellow}0.00{\footnotesize(4.4E+2)} \\
			  
			  \textsc{Sensor} &&&\cellcolor{yellow}1.23{\footnotesize(1.9E+3)}&1.29{\footnotesize(1.4E+3)}\\
			  
			  \textsc{Game} &&&2.41{\footnotesize(1.7E+3)}&\cellcolor{yellow}2.19{\footnotesize(1.4E+3)}\\
			
			  \textsc{Media} &&&2.96{\footnotesize(1.2E+3)}&\cellcolor{yellow}2.90{\footnotesize(1.1E+3)} \\
		

\bottomrule
\end{tabular}
\begin{tablenotes}
    \footnotesize
    \item The better one is highlighted.
\end{tablenotes}
\end{table}
